Better Late than Never; Scaling Computation in Blockchains by Delaying Execution

Proof-of-Work~(PoW) based blockchains typically allocate only a tiny fraction (e.g., less than 1% for Ethereum) of the average interarrival time~($\mathbb{I}$) between blocks for validating transactions. A trivial increase in validation time~($\tau$) introduces the popularly known Verifier's Dilemma, and as we demonstrate, causes more forking and increases unfairness. Large $\tau$ also reduces the tolerance for safety against a Byzantine adversary. Solutions that offload validation to a set of non-chain nodes (a.k.a. off-chain approaches) suffer from trust issues that are non-trivial to resolve. In this paper, we present Tuxedo, the first on-chain protocol to theoretically scale $\tau/\mathbb{I} \approx 1$ in PoW blockchains. The key innovation in Tuxedo is to separate the consensus on the ordering of transactions from their execution. We achieve this by allowing miners to delay validation of transactions in a block by up to $\zeta$ blocks, where $\zeta$ is a system parameter. We perform security analysis of Tuxedo considering all possible adversarial strategies in a synchronous network with end-to-end delay $\Delta$ and demonstrate that Tuxedo achieves security equivalent to known results for longest chain PoW Nakamoto consensus. Additionally, we also suggest a principled approach for practical choices of parameter $\zeta$ as per the application requirement. Our prototype implementation of Tuxedo atop Ethereum demonstrates that it can scale $\tau$ without suffering the harmful effects of naive scaling in existing blockchains.

==> section/analysisRef.tex <==
% !TEX root = ../main.tex
\section{Analysis}
\label{sec:analysisRef}
% We ensured and proved the security of the \prot, which is out of the scope of this paper. Interested readers are motivated to refer our arxiv version~\cite{} for detail.

\prot\ provides security guarantees, equivalent to the known guarantees of the existing PoW system in terms of chain-growth, chain quality, and consistency. \prot\ guarantees this in the presence of a Byzantine adversary under all possible adversarial strategies in a synchronous network with end-to-end
delay of $\Delta$. Proof of which is out of the scope of this paper. Interested readers are motivated to refer to our arxiv version~\cite{tuxedoArxiv} for detail. We also present a principled approach to pick $\ths$ for any given 
choice of parameters in ~\cite{tuxedoArxiv}.
